A Conceptual Framework for Conversational Search and Recommendation: Conceptualizing Agent-Human Interactions During the Conversational Search Process

The conversational search task aims to enable a user to resolve information needs via natural language dialogue with an agent. In this paper, we aim to develop a conceptual framework of the actions and intents of users and agents explaining how these actions enable the user to explore the search space and resolve their information need. We outline the different actions and intents, before discussing key decision points in the conversation where the agent needs to decide how to steer the conversational search process to a successful and/or satisfactory conclusion. Essentially, this paper provides a conceptualization of the conversational search process between an agent and user, which provides a framework and a starting point for research, development and evaluation of conversational search agents.

==> cair-feedbacks.tex <==
----------------------- REVIEW 1 ---------------------
PAPER: 4
TITLE: Conceptualizing Agent-Human Interactions during the Conversational Search Process
AUTHORS: Leif Azzopardi, Mateusz Dubiel, Martin Halvey and Jeffery Dalton

Overall evaluation: 1 (weak accept)

----------- Overall evaluation -----------
I like the overall idea of this paper - it will certainly help researchers to not have to list/think off all those possible actions/intents themselves. At the same time however, the paper is quite weak in terms of its writing and I wonder whether the authors put the right amount of emphasis on the different aspects.

More detailed comments:
- It was not clear to me how the authors' work fits into the prior works that conceptualize (some aspect of) conversational search. While the authors list many papers, they are not very explicit about how their own work works together with the existing literature - are the authors focusing on an aspect that has been ignored so far? Are they breaking down the problems into more concrete steps than prior works? A visualization of how these different works fit together would certainly help.

- Some of the subsections in Section 2 appear overly long; at least I would have liked to see a table that provides a comprehensive overview of all the intents the authors identify. 

- I am not sure that the flight booking example is a good one as a conversational search example, as there is quite a lot of industry emphasis on building domain-specific agents and booking flights is one of the few domains that to my knowledge works at least ok. I would be more interested in an exploratory search example that is more open.

- Section 2.3 was the most interesting to me in terms of potential tasks; sadly, it is the shortest one. Can the authors indicate what kind of ML/IR/NLP techniques could be applicable (as a first try) to solve those tasks?


- Given that most authors are native English speakers, there are a surprising number of spelling and grammar issues, especially in the introduction.


----------------------- REVIEW 2 ---------------------
PAPER: 4
TITLE: Conceptualizing Agent-Human Interactions during the Conversational Search Process
AUTHORS: Leif Azzopardi, Mateusz Dubiel, Martin Halvey and Jeffery Dalton

Overall evaluation: 0 (borderline paper)

----------- Overall evaluation -----------
The paper makes a good attempt at coming up with a set of generalizable terminology to describe the various actions and decision points during a conversational interaction. The authors admit that their work is merely a start and is open to discussion for enhancement and further revision. I am glad that they acknowledge this since the task of coming up generalizable textbook definitions for different intents and states across dialogue systems operating in varied domains is not that easy. These categories and definitions are always going to be up for discussion. E.g. why is "Expand" a new user action type? Why can't it be folded into the "Revise" action with "refine" and "expand" being subtypes. Similarly, should agent actions be categorized into different classes based on the format or amount of information they display/read back? E.g. "list" vs. "summarize". Or is the classification determined by the backend operation necessary for taking the option? So while I agree that th!
e authors have generally done a good job of classifying the most common types of actions and decision points and providing a starting point, I believe a lot of these may always be up for discussion.

More importantly though, as someone who has developed such systems in the industry for the last many years, I fail to see how this kind of classification provides value to a system developer or machine learning engineer building these systems. I am not fully sold on the claim that "the proposed framework would lead to a more principled approach to the design, development and evaluation of agent systems". While the framework is of academic/theoretical interest, building practical applications will always require you to think in concrete terms about the actual task at hand rather than the more abstract notions described here. 

Some comments on improving the text:
- A literary review of the text would definitely help. The language contains typos and other disfluencies, fixing which would help the reader a lot.
- When describing "Recover, Handle and End", you say "these two related actions …" when there are clearly three.
- The background and related work section while useful felt a little like a long enumeration of previous techniques without a lot of discussion/critique on how each one improved or was different from the other.


----------------------- REVIEW 3 ---------------------
PAPER: 4
TITLE: Conceptualizing Agent-Human Interactions during the Conversational Search Process
AUTHORS: Leif Azzopardi, Mateusz Dubiel, Martin Halvey and Jeffery Dalton

Overall evaluation: 2 (accept)

----------- Overall evaluation -----------
This is the meta-review of the paper.

This position paper presents a typology of user actions and agent actions associated with conversational search.  Additionally, the paper describes some of the decision points associated with the agent (and how the agent might be able to inform those decisions).

Overall, the two reviewers saw value in the paper.

Based on the reviews, the paper could be made stronger in several ways.

1. It would be nice to see how the proposed framework relates to existing ones.

2. It would also be useful to present a more concise description of the different user/agent actions and the different decision points (and their associated candidate actions), possibly in a table.

3. I agree with R1 that Section 2.3 (decision points) is the most thought-provoking, and also the 
shortest.

4. As pointed out by R2, it might be good to further explain/justify how a "generalizable framework" 
might be useful to a practitioner working in narrow domain (e.g., online shopping).

5. The writing could benefit from another pass (there are many typos).  Here are some that I found in my own reading of the paper:

Section 1: "for a statement to be rephrases" --> "for a statement to be rephrased".
Section 1: "current state of the coversational" --> "current state of the conversation".
Section 2: "decisions points" --> "decision points".
Section 2: "space options available" --> "space of options available".
